InfiMM-Eval: Complex Open-Ended Reasoning Evaluation For Multi-Modal Large Language Models

Multi-modal Large Language Models (MLLMs) are increasingly prominent in the field of artificial intelligence. These models not only excel in traditional vision-language tasks but also demonstrate impressive performance in contemporary multi-modal benchmarks. Although many of these benchmarks attempt to holistically evaluate MLLMs, they typically concentrate on basic reasoning tasks, often yielding only simple yes/no or multi-choice responses. These methods naturally lead to confusion and difficulties in conclusively determining the reasoning capabilities of MLLMs. To mitigate this issue, we manually curate a benchmark dataset specifically designed for MLLMs, with a focus on complex reasoning tasks. Our benchmark comprises three key reasoning categories: deductive, abductive, and analogical reasoning. The queries in our dataset are intentionally constructed to engage the reasoning capabilities of MLLMs in the process of generating answers. For a fair comparison across various MLLMs, we incorporate intermediate reasoning steps into our evaluation criteria. In instances where an MLLM is unable to produce a definitive answer, its reasoning ability is evaluated by requesting intermediate reasoning steps. If these steps align with our manual annotations, appropriate scores are assigned. This evaluation scheme resembles methods commonly used in human assessments, such as exams or assignments, and represents what we consider a more effective assessment technique compared with existing benchmarks. We evaluate a selection of representative MLLMs using this rigorously developed open-ended multi-step elaborate reasoning benchmark, designed to challenge and accurately measure their reasoning capabilities. The code and data will be released at https://infimm.github.io/InfiMM-Eval/

==> Sec/sec_reasoning.tex <==
\section{Reasoning in LLMs and MLLMs}

\subsection{A brief introduction to reasoning}
\label{sec:reasoning:intro}

Reasoning, a cornerstone of human intelligence, entails the process of comprehending and analyzing information and premises to logically infer new insights~\cite{yu2023nature, huang2022towards, walton1990reasoning}.
In this study, we advocate for a classification of reasoning problems based on directionality, drawing upon established logical frameworks~\cite{bronkhorst2020logical,dowden2018logical}.
Specifically, we focus on deductive, abductive, and analogical reasoning, as these forms are pivotal in the paradigms of human cognitive reasoning.

\noindent\textbf{Deductive reasoning} derives new conclusions from established premises~\cite{johnson1999deductive}, ensures that the steps of inference align with established logical rules.
For example in \figureautorefname~\ref{fig:teaser} deductive example, the premises are ``snow in image'', ``crack is soil after snow melting'' and ``crack is expanding'', the deductive conclusion drawn from premises is ``current season is winter, after winter it will be spring''.

\noindent\textbf{Abductive reasoning} ascertains the most plausible explanation based on common sense for a given set of observations \cite{douven2011abduction}, which is often considered the inverse of deductive reasoning.
For instance, in \figureautorefname~\ref{fig:teaser} abductive example, based on observation ``a person is cutting onion with a helmet'', common sense ``Onions can release compound that make eyes irritate'', the most plausible explanation for the question is to ``protect eyes''.

\noindent\textbf{Analogical reasoning} enables transfer knowledge from known instances to similar situations \cite{goswami1991analogical}. 
In \figureautorefname~\ref{fig:teaser} analogical example, the first image reveals the proposition that the naming convention is a play on words involving depth. The second and third images should follow similar pattern. The person in second image faces east, in third image faces west, thus his name should be ``Westface''.

\subsection{Reasoning in MLLMs}
LLMs have demonstrated significant capabilities in reasoning across a range of NLP tasks, as evidenced by recent studies ~\cite{kojima2022large,huang2022towards,wei2022emergent,yao2022react,webb2023emergent}.
Similar reasoning abilities in MLLMs have also been observed~\cite{driess2023palm,gpt4systemcard}.
However, MLLMs research field lacks systematic categorization of reasoning capability. 
For example, recent MLLM benchmarks categorize reasoning abilities as common sense reasoning, math reasoning, code understanding, relation reasoning, action prediction, procedure understanding etc. Such task specific reasoning ability categorization will create hundreds of reasoning tasks, hinder people's understanding about MLLMs' general reasoning capability, thus cannot improve reasoning capability from the root.

To shed the light on better understanding MLLMs reasoning capability, following previous discussion, we propose to categorize MLLM reasoning ability into deductive, abductive and analogical.
These 3 reasoning types covers a wide range of tasks and applications.
Deductive reasoning capability is crucial for MLLMs in the field of automatic fact-checking (verify accuracy of multimodal information), multimodal legal reasoning (deduce legal interpretations or judgments with multimodal legal documents), etc. 
Abductive reasoning capability can be used for causal inference in complex systems, like economic data combined with news reports infer public sentiment or predict trends by analyzing textual posts alongside images and videos. 
Analogical reasoning capability is useful for comparative analysis, which is the key to in context learning.
Recognizing the broad scope and practical applicability of this categorization of reasoning, we aim to develop a multimodal reasoning benchmark that focuses on these three reasoning types. This benchmark is designed to facilitate a thorough and comprehensive assessment of MLLMs' reasoning capabilities.

==> preamble.tex <==
%
% --- inline annotations
%
% \usepackage[dvipsnames]{xcolor}
% \newcommand{\red}[1]{{\color{red}#1}}
% \newcommand{\todo}[1]{{\color{red}#1}}
% \newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


